Capital as Artificial Intelligence

We gather many perspectives on Capital and synthesize their commonalities. We provide a characterization of Capital as a historical agential system and propose a model of Capital using tools from computer science. Our model consists of propositions which, if satisfied by a specific grounding, constitute a valid model of Capital. We clarify the manners in which Capital can evolve. We claim that, when its evolution is driven by quantitative optimization processes, Capital can possess qualities of Artificial Intelligence. We find that Capital may not uniquely represent meaning, in the same way that optimization is not intentionally meaningful. We find that Artificial Intelligences like modern day Large Language Models are a part of Capital. We link our readers to a web-interface where they can interact with a part of Capital.

==> background.tex <==
§0.02 — Economies are assembled from flows. Unsurprisingly, therefore, their native codes are currencies, or current-signs. As societies mobilize matter-energy resource streams, their monetary conventions register these flows by inversion, and strict reciprocity. Hole-flow in electronics is a close analog. Every non-barter commodity exchange, or non-financial transaction, catalyzes a flow, by pricing it. The ‘real economy’ is thus automatically captured, by a monetary code, even when – as is overwhelmingly typical – this quantification through signs is never aggregated. Since money systems install an intrinsic economic intelligence (preceding all reflective theorization), economics – uniquely among the sciences – inherits a field of objectivity whose arithmetization has already taken place. This same delicate shadow, cast into business ledgers (pre-denominated by currencies), at once facilitates and registers a system of flows, in a twin production of economic objects. Business is recorded in the way it is produced. Dynamization of the commodity – or economic circulation – is not reducible to, but nevertheless strictly corresponds to, transference of signs.


§0.211 — Critique – the critique of metaphysics – is philosophy (as a current undertaking). It is what philosophy has irreversibly become. Insofar as these terms still diverge, however minutely, there is a task that remains uncompleted. Philosophy establishes itself in modernity by way of auto-critique. ‘Like’ Capital it is a path with firm direction, but without destination (the path is the destination). It exists only by perpetually overcoming itself. Critical – or diagonal – method is a tool through which philosophy is definitively exhausted. Its sole product is immanence. The rigorously complementary formulation asserts: Residual transcendence is the negative of the philosophical undertaking. The systematization of the synthetic a priori is the model of diagonalization in philosophy. Bitcoin is therefore in the very strictest sense a critical enterprise, targeting “trusted third parties” as superfluous metaphysical structures. Immanence is its techonomic – or socio-historical – rather than its merely reflective-conceptual output (or production).


§0.531 — Money thinks. In fact, it out-thinks us, insofar as reflection is brought to it late, after its own cognitive operation has been long at work, and ultimately perhaps also in other ways, yet to be apprehended (from our side). It has already made sense of things, before we have begun to make sense of it. We have no grounds upon which to affirm, with confidence, that money and general intelligence can be finally distinguished. The institutional separation between artificial intelligence research and crypto-currency innovation is not rooted in philosophical principle.[22] The expectation that catallaxy, distributed commercial learning, or price discovery encounters a limit short of the question of the price of being finds its sole resilient foundation in moral indignation. Since Bitcoin demonstrably does ontology, and even ‘fundamental ontology’, the status of normative revulsion in this domain is irredeemably dubious.

§1.31 — Since the origins of modernity, a specter has been haunting the world – that of the autonomous industrial economy. This is the same emergent order that has acquired the name ‘capitalism’ in the abstract, tendential, or teleological sense of the word, and – still more importantly – in accordance with its usage as a designation for an always only partially-defined real individual, or terrestrial event. Its signature is a regenerative, or self-reinforcing, intensification of socio-economic disequilibrium, ‘governed’ – or, more strictly, made radically ungovernable – by a fundamental positive-feedback dynamic. ‘Capitalism’ then, as a singular (or ‘proper’) rather than generic (or typological) name, designates the sovereign self-escalation of an innovative entity, defined only by the practical relation of auto-promotion it establishes with – and through – itself. What it is, in itself, is more than itself. Growth is its essence. This is easily said, but – as an irreducible logical anomaly – it is far less easily understood. This does not, however, obstruct its being named. Fernand Braudel writes of “the passionate disputes the explosive word capitalism always arouses.”[39] Its would-be defenders, typically, are those least inclined to acknowledge its real (and thus autonomous) singularity. Business requires no such awkward admission. This, too, is a crypsis. By inevitable – if often awkward – irony, a species of ‘Marxism’ tends to be regenerated in any systematic promotion of Capital. Even were this not the case, those who consider themselves befriended by Capital would rarely be motivated to pronounce upon the fact.

Capital is essentially capitals, at war among themselves. It advances only through disintegration. If – not at all unreasonably – the basic vector of capital is identified with a tendency to social abandonment, what it abandons most originally is itself.

47. Fernand Braudel’s great study of Civilization \& Capitalism includes an illuminating survey of the energy resources commanded by human civilizations in the period immediately antecedent to modernity. The linchpin of energy abstraction – or plasticity – was man, conceived as a source of mechanical power. On the basis of his unmatched versatility, human laboring effort would remain the critical energy transformer until far into the 19th century. Secondary only to man himself in flexibility was the supplementary work of animals, typically bred for specific functions, but available for limited redeployment. Alongside men, a range of other laboring animals – mules, oxen, camels, and horses – converted nutritional calories into work. In Europe, especially, horses occupied an especially privileged place, as reflected by the persistence of ‘horse-power’ as a measure of quantitative industrial effort – i.e. power, or work rate. The metric was introduced by James Watt in the late 18th century, and – by neat historical symmetry – it was the ‘watt’ as an electrical measure of power that would much later displace horsepower from its technical centrality. The only sources of energy available from non-agricultural sources were wind and water, predominantly in the sails of nautical vessels, but also very significantly in the large numbers of mills that composed the earliest mechanical energy infrastructure. Crucially, these power resources were not convertible into a general (or abstract) form. Retrospectively, it is tempting to assign some such role to wood and charcoal, but this is unconvincing due to the very limited range of industrial applications for combustion prior to the switch to coking coal (and the first steam-powered mills). It is only with the ‘industrial revolution’ brought by steam power that a fungible stock of fuel – and thus standardized energy reserves – became available as a comparatively general-purpose power source, of very broad mechanical application. The introduction of the electric turbine represents a technical subsumption of this first industrial energy infrastructure into one of far superior abstraction. All sources of energy supply, when applied to the generator as an intermediate machine, are pooled into a single power reservoir of at least tendential homogeneity. Lenin’s widely-cited definition of communism as “Soviet power plus the electrification of the whole country” appears in context as an empirical-pragmatic – and even nakedly opportunistic – slogan, lending itself to an apprehension of electricity as a socio-political resource, essentially incapable of rising to the level of serious philosophical consideration (thus eliciting a certain condescending humor within the subsequent development of Western Marxism). Yet even in this account, the order of emphasis is sufficient to mark out electricity as a practical abstraction, or fungible resource, whose facilitation of energy quantification at an unprecedented level advances its ‘commoditization’ (in the mainstream economic, rather than specifically Marxian sense). See V. I. Lenin ‘Our Foreign and Domestic Position and Party Tasks’ (November 21, 1920). 

Electrification and then electronics are decisive thresholds in its course. New units of abstract power, and of information, are indices of irreversible submission, folding the concrete apparatus of production and transmission into an activated system from which there can be no retreat. The system – in each case – is in a very real sense nothing but its parts, but it was not before, and now is, and there is no going back.

What a system is, isn’t anything in particular, at all. Rather, a system is that which remains – by necessity excluded – even after a comprehensive enumeration of parts. Any real system is an irreducible individual, a true ‘thing’.[50] Critically, individuality is a scale-free concept, assigning reality to an object. It summarizes a meta-stable knot of connectivity, or synthesis. When formulated as a critical proposition: the systematicity of the system is irreducible to any part or parts of the system.

Bitcoin is a machine.[57] More specifically, it is a credibility machine. Its ideal operation coincides with the most rigorous realizable definition of truth. That is already to assert everything. In particular, it proposes that there are no (conceivably reachable) grounds of truth which offer leverage in respect to the Bitcoin protocol.

  57. Bitcoin is a machine in the literal but non-reductive sense that the Internet, planetary capitalism, or the terrestrial biosphere are machines – which is to say that it is a distributed productive assemblage. It is not, of course – to employ the distinction Deleuze \& Guattari insist upon – a mere gadget. The difference is strictly critical, based upon an apprehension without reference to transcendence. The immanence of the machine, in contrast to the gadget, is determined by an auto-production: it functions in the same way it is produced. Within the industrial process, circuits of mechanical reproduction are typically too highly-ramified to isolate with confidence. In Bitcoin the circuit of auto-production is manifested with unprecedented, compact definition. Graphically – diagrammatically – it is governed in the same way it is industrially generated. As an exemplary machine, and unlike a gadget, there is no difference between how it operates and the way it is made. 

  

§2.56 — Although the world is probably not yet ready for the question of the price of Being, if it ever will be, its most fundamental ontological problems are bound to the fate of a digital currency system, nevertheless. The intrinsic abstraction of money is not obviously delimitable. To twist a Spinozistic formulation: We do not know what money can do. The process of monetary sophistication, which is by no means restricted to ‘financialization’ in its contemporary sense, automatically projects a convergence of money and intelligence as it tends to the monetization of general-purpose problem-solving (by subjecting it to the discipline of price-discovery). Crypto-digital currency inclines to the distributed production of a synthetic cognitive medium, attesting to the primordial complicity of Capital teleology with the production of artificial intelligence. Within the industrial social order (capitalism), markets manifestly – and consistently – drive the production of intelligent machines. Modernity demonstrates no stronger trend. (Theoretical expectation supports this proposition no less firmly than empirical evidence.[80])

 80. Since political economy is essentially torn by ideological conflict it provides only unstable support for general conceptual definitions. Were this not the case, it would be impossible to find a superior locus for the rigorous determination of intelligence than the techonomic matrix. What defines intelligence most essentially is general-purpose industrial capability, the precursor to which is anticipated by animal brains, among other biological systems. The market process is the transcendental criterion for evaluating (‘pricing’) this supreme synthetic resource. To second guess its judgment is exactly to succumb to the calculation problem (as Mises classically outlines it). Within the arena of ideological controversy, this proposition can expect dismissal for its ‘circularity’. Of course, it is circular (which is only to say: self-grounding, cybernetic, immanent, or critical). 



§2.34 — It is from irreversibility – of the one-way (or ‘trap-door’) crypto-function, the thermodynamic gradient, and ultimately of absolute time – that the reliable principle of analytic-synthetic distinction can be isolated. A mathematical proof is easier to confirm than to construct. Prime numbers are easily multiplied, but their product is time-consuming to factorize. Bitcoin blocks are easy to check, but hard to mine. In each case there is a distinction between analytical facility and (comparative) synthetic intractability. When cryptographically re-conceived, analysis and synthesis co-produce a ratchet. Adam Back (on Twitter) describes the mechanized contractual commitment that exploits this gradient as “computational irrevocability”. Like a carnivorous plant, it is easy to enter, but then difficult to escape. History is a Venus flytrap, self-abstracted beyond botany.


That which most incontestably demonstrates its resilience – by enduring into the future ¬– is the past. What has happened, alone, is realized.

Among Austrian Schools economists, objective price arises solely from the catallactic interplay of subjective preferences, while among Bayesian probabilists, objectivity in estimation is achievable only through the rational updating of subjective ‘priors’, to mention only two critical examples. The subjective stance in such cases is not a dogmatic commitment, but rather the opposite. It is a skeptical suspension, corresponding to the status of objectivity as a production. Subjectivity is work not yet done. That which has not been earned, in respect to an attribution of reality, falls automatically onto the side of subjectivity.

Capital is the growth of abstract value.


\cite{land2018crypto}

Without attachment to anything beyond its own
abysmal exuberance, capitalism identifies itself
with desire to a degree that cannot imaginably be
exceeded, shamelessly soliciting any impulse that
might contribute an increment of economisable drive
to its continuously multiplying productive initiatives.
Whatever you want, capitalism is the most reliable
way to get it, and by absorbing every source of social
dynamism, capitalism makes growth, change and
even time itself into integral components of its endlessly gathering tide. 'Go for growth' now means 'Go
(hard) for capitalism ' .

Capitalism [ . . . ] has no external limit, it has consumed
life and biological intelligence to create a new life
and a new plane of intelligence, vast beyond human
anticipation. The Transcendental Miserabilist has
an inalienable right to be bored, of course. Call this
new? It's still nothing but change .

Life continues, and capitalism does life in a way it has
never been done before. If that doesn't count as 'new ' ,
then the word 'new' has been stripped down to a hollow
denunciation.
\cite{land2011critique}

As capital 'evolves', the increasingly
absurd rationalization of production-for-profit peels away
like a cheap veneer from the positive-feedback detonation
of production-for-production.
\cite{land1988kant}

Capital propagates virally in so far as money
communicates addiction, replicating itself through host
organisms whose boundaries it breaches, and whose
desires it reprograms. It incrementally virtualizes production; demetallizing money in the direction of credit
finance, and disactualizing productive force along the
scale of machinic intelligence quotient. The dehumanizing
convergence of these tendencies zeroes upon an integrated
and automatized cyberpositive techno-economic intelligence at war with the macropod.
\cite{land1993machinic}

Capitalism's like
an organism . right? . . . but an organism that's evolved
much too fast to develop a reliable immune system . . . 
\cite{land2011cyberrevolution}

"But capital has one single life impulse, the tendency to create value and surplus-value, to make its constant factor, the means of production, absorb the greatest possible amount of surplus-labour."

"Capital is dead labour, that, vampire-like, only lives by sucking living labour, and lives the more, the more labour it sucks." \cite{marx2004capital}

Workers get paid for working; what do capitalists get paid for? For 'waiting' while roundabout processes of production percolate, or for 'abstaining' from some current consumption in favor of replacing or augmenting the stock of capital and maintaining or increasing future consumption. \cite{solow1963capital}

A man from Mars reading the literature on capital theory would be inclined sometimes to think that capital consists mainly of stocks of consumer goods to maintain workers until their output can be sold; sometimes he would think that the earth is given over to the maturing of wine and the growing of trees, so that capital consists largely of goods in process; sometimes he would realize that most of what we think of as capital consists of durable assets like buildings and machinery, or what we call fixed capital. He would perhaps wonder why Wicksell, in the course of a careful analysis of a model with fixed capital in the form of axes, did not pay any attention to the age of the trees being cut down (though he had done so 30 years earlier), whereas Bohm-Bawerk, who seemed to be thinking mainly about the age at which trees should be cut down, seemed to worry too little about the implement to be used in felling them. He would be a little uncertain whether gestation periods matter a lot or not, whether production is like making elephants or making mosquitoes. The truth, of course, is that all these aspects of capitalistic production are important, that it is useless to try to represent all of them by any one of them, and extraordinarily complicated to deal simultaneously with them all. \cite{solow1963capital}

without a satisfactory account of behavior under uncertainty we cannot have a complete theory of capital. \cite{solow1963capital}

Despite their pivotal significance, the definition of capital and the meaning of accumulation have remained unsettled (Schumpeter 1954: 322-327, 625-645; Braudel 1982: 232-249). Historically, the principal contention stemmed from trying to marry two different perceptions of capital: one as an income generating fund, or 'financial wealth', the other as a stock of physical instruments, or 'capital goods' (pasinetti and Scazzieri 1987). The central question has been whether and in what way 'capital goods' are productive, and how their productivity affects their overall magnitude as 'capital' (Hennings 1987). Mainstream economics has generally tried to show that capita,! goods were indeed productive, and that this 'positive' attribute is what made .capital as a 'fund' valuable. \cite{nitzan2000capital}

"Secondly, and this is even more important, the attempts to explain interest, by analogy with wages and rent, as the price of the services of some definitely given "factor" of production, has nearly always led to a tendency to regard capital as a homogeneous substance the "quantity" of which could be regarded as a " datum", and which, once it had been properly defined, could be substituted, for purposes of economic analysis, for the fuller description of the concrete elements of which it consisted. It was inevitable in these circumstances that different authors should have singled out different aspects of the same phenomenon as the relevant ones, and the consequences of this were those unending discussions about the "nature" of capital which are among the least edifying chapters of economic science."

"The problems that are raised by any attempt to analyse the dynamics of production are mainly problems connected with the interrelationships between the different parts of the elaborate structure of productive equipment which man has built to serve his needs. But all the essential differences between these parts were obscured by the general endeavour to subsume them under comprehensive definition of the stock of capital. The fact that this stock of capital is not an amorphous mass but possesses a definite structure, that it is organised in a definite way, and that its composition of essentially different items is much more important than its aggregate "quantity", was systematically disregarded. Nor did it help much further when it was occasionally emphasised that capital was an " integrated organic conception"1, so long as such hints were not followed up by a careful analysis of the way in which the different parts were made to fit together."

"The problem takes on a different complexion, however, as soon as we ask how a state of stationary equilibrium can ever be brought about, or what will be the reaction of a given system to an unforeseen change. It is then no longer possible to treat the different aspects of capital as one, and it becomes evident that the "quantity of capital" as a value magnitude is not a datum,l but only a result, of the equilibrating process. With the disappearance of stationary equilibrium capital splits into two different entities whose movements have to be traced separately and whose interaction becomes the real problem. There is no longer one supply of a single factor, capital, which can be compared with the productivity schedule of capital in the abstract: and the terms demand and supply, as referring to magnitudes which affect the rate of interest, take on a new meaning. It is the existing real structure of productive equipment (which in long-term equilibrium is said to represent the supply) which now determines the demand for capital; and to describe what constitutes the supply, writers have usually been compelled to introduce such vague and usually undefined terms as "free" or "disposable" capital."
\cite{hayek2019pure}


\section{Outline}

Capital is alive. Much like a human being, which is an aggregation of a multitude of parts, many of which are alive and have significant autonomy, Capital also emerges out of the interactions of independent parts. 

In simple terms life may be seen minimally as the information carried by the genetic code and matter/energy that processes it. In these terms Capital is also information in the form of currency and the matter/energy that it consumes ("Capital is dead labour, that, vampire-like, only lives by sucking living labour, and lives the more, the more labour it sucks." \cite{marx2004capital}). It is an essentially historic process that acts, by the mediation of symbols, to assign and quantify its environment under a common denominator.

According to the autopoietic definition of life Capital is alive because it produces and maintains itself by creating its own parts. It is a self-recurrent feedback process that accounts for itself and thus is able to continue.     

According to the functional definition capital could also be considered alive as it exhibits properties such as: homeostasis, organisation, metabolism, growth, adaptation, response to stimuli (requires some further linkage and explaining). 

All in all, it has been common place to anthropomorphise Capital, to ascribe it life-like qualities and agency (Marx, Land, Hayek). While we intend to provide strong arguments for why it is reasonable to consider Capital as alive, we make a point that at the very least it can be seen as alive by analogy (as substantiated by the language used in literature). 

It therefore seems that capital being an artificial system that is alive would be a perfect object of study for the Artificial Life community. 

In this work we propose an agent model of the capital that we refer to as the Capital Agent. The capital is modeled through continuous reinforcement learning (note the potent biological inspiration behind rl). 

Capital, like all life, needs energy from the outside. Biological life siphons energy from its environment (sunlight) and uses it to decrease its own entropy. But what is outside of Capital. At the current stage, Capital siphons some of this energy from the future. Capital also uses this energy to decrease its own information entropy. 

“The simple circulation of commodities – selling in order to buy – is a means of carrying out a purpose unconnected with circulation, namely, the appropriation of use-values, the satisfaction of wants. The circulation of money as capital is, on the contrary, an end in itself, for the expansion of value takes place only within this constantly renewed movement. The circulation of capital has therefore no limits.” [Capital, Chapter 4]

“In order to be able to extract value from the consumption of a commodity, our friend, Moneybags, must be so lucky as to find, within the sphere of circulation, in the market, a commodity, whose use-value possesses the peculiar property of being a source of value, whose actual consumption, therefore, is itself an embodiment of labour, and, consequently, a creation of value. The possessor of money does find on the market such a special commodity in capacity for labour or labour-power.” [Capital, Chapter 6]

"Labor is not the source of all wealth. Nature is just as much a source of use values (and it is surely of such that material wealth consists!) as labor, which is itself only the manifestation of a force of nature, human labor power.[54]"

According to Marx Capital arises from the surplus value created via labour. Historically the emergence of surplus value is associated with the beginning of civilisation (~10000BC), where the surplus value would be created by applying novel agrarian technologies. The pre-agrarian hunter-gatherer societies do not have a concept of wage labour because they do not have currency. Thus they cannot exchange or accumulate abstract value.

“Technique is the totality of methods, rationally arrived at and having absolute efficiency (for a given stage of development) in every field of human activity.”
Ellul, the Technological Society 

"Modern technology has become a total phenomenon for civilization, the defining force of a new social order in which efficiency is no longer an option but a necessity imposed on all human activity."
Ellul

It fell to the modern commodity producing system as an end-in-itself with its ceaseless transformation of human energy into money to bring about a separated sphere of so-called labour “alienated” from all other social relations and abstracted from all content. It is a sphere demanding of its inmates unconditional surrender, life-to-rule, dependent robotic activity severed from any other social context, and obedience to an abstract “economic” instrumental rationality beyond human needs. In this sphere detached from life, time ceases to be lived and experienced time; rather time becomes a mere raw material to be exploited optimally: “time is money”. Any second of life is charged to a time account, every trip to the loo is an offence, and every gossip is a crime against the production goal that has made itself independent. Where labour is going on, only abstract energy may be spent. Life takes place elsewhere – or nowhere, because labour beats the time round the clock. Even children are drilled to obey Newtonian time to become “effective” members of the workforce in their future life. Leave of absence is granted merely to restore an individual’s “labour power”. When having a meal, celebrating or making love, the second hand is ticking at the back of one’s mind.
Manifesto against labour

\textbf{Motivation}
\begin{itemize}
    \item not many examples of actual ALIFE
    \item Capital is an alive artificial system
    \item Not present in ALIFE community
    \item Many have suggested it is alive/organism/agent
    \begin{itemize}
        \item but not properly claimed
        \item many perspectives/political origins
    \end{itemize}
    \item provide a formal model
\end{itemize}

\section{Background}

\textbf{Background}
\begin{itemize}
    \item Themes: autopoiesis, complex systems, information/entropy, organism, agential entity, invisible hand, self-organization, anthropomorphism, history dependence
    \item Nick Land, Adam Smith, Marx, Hayek, Biel
    \item Traditional economics and incompatibilities, e.g. static systems, Keynes, efficient markets
\end{itemize}

\textbf{Principles}
\begin{itemize}
    \item distill key `axioms'
    \item write them in Reinforcement Learning Language
\end{itemize}

\textbf{Use cases and interpretation}
\begin{itemize}
    \item create AI agents which behave `like capital'
    \item conceptualized the role of individuals, groups within capital
\end{itemize}
